ReGen: Zero-Shot Text Classification via Training Data Generation with Progressive Dense Retrieval

With the development of large language models (LLMs), zero-shot learning has attracted much attention for various NLP tasks. Different from prior works that generate training data with billion-scale natural language generation (NLG) models, we propose a retrieval-enhanced framework to create training data from a general-domain unlabeled corpus. To realize this, we first conduct contrastive pretraining to learn an unsupervised dense retriever for extracting the most relevant documents using class-descriptive verbalizers. We then further propose two simple strategies, namely Verbalizer Augmentation with Demonstrations and Self-consistency Guided Filtering to improve the topic coverage of the dataset while removing noisy examples. Experiments on nine datasets demonstrate that REGEN achieves 4.3% gain over the strongest baselines and saves around 70% of the time compared to baselines using large NLG models. Besides, REGEN can be naturally integrated with recently proposed large language models to boost performance.

==> 01-intro.tex <==




==> 02-exp.tex <==
\begin{table*}[!t]
% \resizebox{\linewidth}{!}{%
% \scalebox{0.57}{
\centering 
\renewcommand\arraystretch{0.86}
\fontsize{7.5}{9.5}\selectfont \setlength{\tabcolsep}{0.5em}
\resizebox{0.98\linewidth}{!}{%
\begin{tabular}{l|ccccc|cccccc|c}
\toprule
\bf    Task ($\rightarrow$)     & \multicolumn{5}{c|}{\textbf{Topic Classification}}  &  \multicolumn{6}{c|}{\textbf{Sentiment Classification}} & \bf All  \\  \hline   
\bf    Method ($\downarrow$) / Dataset ($\rightarrow$)    & \bf  AG News & \bf DBPedia & \bf Yahoo  & \bf NYT & \multicolumn{1}{>{\columncolor{maroon}}c}{\bf Avg.} & \bf  IMDB & \bf MR & \bf SST-2 & \bf Amazon  & \bf Yelp &  \multicolumn{1}{>{\columncolor{lightblue}}c}{\bf Avg.} & \multicolumn{1}{>{\columncolor{yellow}}c}{\bf Avg.} \\ \hline
\multicolumn{10}{l}{\emph{Zero-shot Learning via Direct Inferencing on Test Data}}  \\\hline 
Dataless~\shortcite{dataless} & 69.6 & 63.4 & 40.4 & 44.2	& \multicolumn{1}{>{\columncolor{maroon}}c}{59.4} & 50.5 & 55.2 & 52.2 & 52.8 &  51.1 &  \multicolumn{1}{>{\columncolor{lightblue}}c}{52.4} & \multicolumn{1}{>{\columncolor{yellow}}c}{55.9}	\\
NSP-BERT~\shortcite{sun2021nsp} & 78.1 & 69.4 & 47.0 & & \multicolumn{1}{>{\columncolor{maroon}}c}{} & & 74.4 & 75.6 & & &  \multicolumn{1}{>{\columncolor{lightblue}}c}{} \\ 
Prompt~\shortcite{van2022don} & 34.0 & 36.4 & 28.2 & --- & \multicolumn{1}{>{\columncolor{maroon}}c}{---}  & 78.4 & 71.1 & 77.4 & 81.5  & 81.9 & \multicolumn{1}{>{\columncolor{lightblue}}c}{78.0}  & \multicolumn{1}{>{\columncolor{yellow}}c}{---}  \\
Prompt (\emph{Our ReImp.}) & 73.2 & 71.3 & 44.1 & 57.4 & \multicolumn{1}{>{\columncolor{maroon}}c}{61.5}  &  74.8 & 73.2 & 75.9 & 80.2 & 78.1 & \multicolumn{1}{>{\columncolor{lightblue}}c}{76.4}  & \multicolumn{1}{>{\columncolor{yellow}}c}{68.9}  \\
KNN-Prompt~\shortcite{shi2022nearest} & 78.8 & --- & 51.0 & --- & \multicolumn{1}{>{\columncolor{maroon}}c}{---}  &  --- & 78.2 & 84.2 & 85.7 & --- & \multicolumn{1}{>{\columncolor{lightblue}}c}{---} & \multicolumn{1}{>{\columncolor{yellow}}c}{---} \\
GPT-3$^\ddagger$~\shortcite{zhao2021calibrate} & 73.9 & 59.7 & 54.7 & 57.0 & \multicolumn{1}{>{\columncolor{maroon}}c}{61.3}  & 75.8 & 76.3 & 87.2 & 75.0 & 78.5 & \multicolumn{1}{>{\columncolor{lightblue}}c}{78.6} & \multicolumn{1}{>{\columncolor{yellow}}c}{69.9} \\
\hline
\multicolumn{10}{l}{\emph{Zero-shot Learning via Generating Task-specific Datasets}} 
 \\\hline
LOTClass$^{\natural}$~(\emph{Our ReImp.}) & & & & &  \multicolumn{1}{>{\columncolor{maroon}}c}{---}  & \\
SuperGen$^\ddagger$~\shortcite{meng2022generating} & 77.4\std{1.5} & 66.5\std{2.0} & 40.8\std{1.5}& 53.9\std{1.5} & \multicolumn{1}{>{\columncolor{maroon}}c}{59.7} & 85.8\std{1.6} & 81.9\std{0.9} & 88.6\std{0.5} & 91.0\std{0.9} & \bf  93.6\std{0.6} &  \multicolumn{1}{>{\columncolor{lightblue}}c}{88.1} & \multicolumn{1}{>{\columncolor{yellow}}c}{73.9}
\\
Mining$^*$~\shortcite{van2022don} & 79.2 & 80.4 & 56.1 & --- & \multicolumn{1}{>{\columncolor{maroon}}c}{---} & 86.7 & 80.5 & 85.6 & 92.0 & 92.0 & \multicolumn{1}{>{\columncolor{lightblue}}c}{87.3} & \multicolumn{1}{>{\columncolor{yellow}}c}{---}\\
Mining$^{*\natural}$ (\emph{Our ReImp.}) & 79.7\std{1.0} & 82.1\std{0.6} & 57.0\std{0.6} & 68.6\std{0.9} & \multicolumn{1}{>{\columncolor{maroon}}c}{71.9}  &
87.1\std{0.6}  & 79.9\std{0.7} &  85.0\std{0.6} & 92.1\std{0.5} & 92.3\std{0.5} & \multicolumn{1}{>{\columncolor{lightblue}}c}{87.2} & \multicolumn{1}{>{\columncolor{yellow}}c}{79.6}\\
\hline
\bf {\ours}  (Our Method) & \bf{85.2\std{0.8}} & \bf 88.0\std{0.9}& \bf  59.5\std{0.8} & \bf  74.5\std{1.1} & \multicolumn{1}{>{\columncolor{maroon}}c}{\bf 76.8}  & \bf  89.9\std{0.5} & \bf  82.5\std{0.7} & \bf  88.9\std{0.4} & \bf  92.3\std{0.4} &  93.0\std{0.5} & \multicolumn{1}{>{\columncolor{lightblue}}c}{\bf 89.3} & \multicolumn{1}{>{\columncolor{yellow}}c}{83.0}\\
\hline
% \hline
% $\text{}^{\sharp}$
% \midrule
%% *********************************************************************
\multicolumn{10}{l}{\emph{\textbf{For Reference Only}: Using larger models / labeled data from other tasks / task-specific corpus / external knowledge base.}}  
\\ \hline
TE-NLI (Best)$^\dagger$~\shortcite{yin-etal-2019-benchmarking} & 78.0 & 73.0 & 43.8 & 70.7 & \multicolumn{1}{>{\columncolor{maroon}}c}{66.4}  & 64.6 & 68.3  & 68.6 & 76.7 & 73.5 &  \multicolumn{1}{>{\columncolor{lightblue}}c}{70.3} & \multicolumn{1}{>{\columncolor{yellow}}c}{68.6} \\
NATCAT$^\dagger$~\shortcite{chu2021natcat} & 68.8 &  81.9 & 57.8 & 42.0 & \multicolumn{1}{>{\columncolor{maroon}}c}{62.6}  & 54.0 & 51.0 & 65.0 & 66.8 & 75.2 &  \multicolumn{1}{>{\columncolor{lightblue}}c}{62.4} & \multicolumn{1}{>{\columncolor{yellow}}c}{62.5}\\
KPT$^{\sharp,\S}$~\shortcite{hu-etal-2022-knowledgeable} & 84.8 & 82.2  & 61.6 & 72.1 &\multicolumn{1}{>{\columncolor{maroon}}c}{75.2}  & 91.2 & --- & --- & 92.8 & --- &  \multicolumn{1}{>{\columncolor{lightblue}}c}{---} & \multicolumn{1}{>{\columncolor{yellow}}c}{---} \\
LOTClass$^\sharp$~\shortcite{meng-etal-2020-text} & 86.2 & 91.1 & 55.7 & 49.5 & \multicolumn{1}{>{\columncolor{maroon}}c}{70.7}  & 86.5 & 68.8 & 74.9 & 91.6 & 87.6 & \multicolumn{1}{>{\columncolor{lightblue}}c}{81.9} & \multicolumn{1}{>{\columncolor{yellow}}c}{76.3} \\
X-Class$^\sharp$~\shortcite{wang-etal-2021-x} & 85.7 & 91.3 & 50.5 & 68.5 & \multicolumn{1}{>{\columncolor{maroon}}c}{74.0}  &  &  &  & 90.2 & 90.0 & \multicolumn{1}{>{\columncolor{lightblue}}c}{} & \multicolumn{1}{>{\columncolor{yellow}}c}{} \\
%  \midrule
\bottomrule
\end{tabular}
}
\vspace{-0.8ex}
\caption{Main results. We report average performance and standard deviation across 5 runs \emph{only if fine-tuning is applied}. $*$: concurrent work, $\natural$: use the same corpus and template as {\ours} for \emph{fair comparison}, $\dagger$: use labeled data from auxiliary tasks, $\sharp$: use task-specific corpus,  $\ddagger$: use billion-scale PLMs, $\S$: use additional knowledge base.}
\label{tab:main_f1}
% }
\vspace{-1.5ex}
\end{table*}


